A Survey of Large Language Models Attribution

Open-domain generative systems have gained significant attention in the field of conversational AI (e.g., generative search engines). This paper presents a comprehensive review of the attribution mechanisms employed by these systems, particularly large language models. Though attribution or citation improve the factuality and verifiability, issues like ambiguous knowledge reservoirs, inherent biases, and the drawbacks of excessive attribution can hinder the effectiveness of these systems. The aim of this survey is to provide valuable insights for researchers, aiding in the refinement of attribution methodologies to enhance the reliability and veracity of responses generated by open-domain generative systems. We believe that this field is still in its early stages; hence, we maintain a repository to keep track of ongoing studies at https://github.com/HITsz-TMG/awesome-llm-attributions.

==> figures/taxonomy_xs.tex <==
\tikzstyle{my-box}=[
    rectangle,
    draw=light-blue,
    rounded corners,
    text opacity=1,
    minimum height=1.5em,
    minimum width=5em,
    inner sep=2pt,
    align=center,
    fill opacity=.5,
    line width=0.8pt,
]
\tikzstyle{leaf}=[my-box, minimum height=1.5em,
    fill=hidden-pink!80, text=black, align=left,font=\normalsize,
    inner xsep=2pt,
    inner ysep=4pt,
    line width=0.8pt,
]
\begin{figure*}[t!]
    \centering
    \resizebox{\textwidth}{!}{
        \begin{forest}
            forked edges,
            for tree={
                grow=east,
                reversed=true,
                anchor=base west,
                parent anchor=east,
                child anchor=west,
                base=left,
                font=\large,
                rectangle,
                draw=light-blue,
                rounded corners,
                align=left,
                minimum width=4em,
                edge+={darkgray, line width=1pt},
                s sep=3pt,
                inner xsep=2pt,
                inner ysep=3pt,
                line width=0.8pt,
                ver/.style={rotate=90, child anchor=north, parent anchor=south, anchor=center},
            },
            where level=1{text width=7em,font=\normalsize,}{},
            where level=2{text width=8.5em,font=\normalsize,}{},
            where level=3{text width=8em,font=\normalsize,}{},
            where level=4{text width=5em,font=\normalsize,}{},
            [
                Large Language Models Attribution, ver, fill=light-yellow
                [
                    Sources (\S \ref{sec:Sources_of_Attribution}), fill=light-green
                    [
                        Pre-training \\Data  (\S \ref{sec:Pre-training_Data}), fill=light-skyblue
                        [
                            ORCA~\cite{DBLP:journals/corr/abs-2205-12600}{, }
                            ORCA-ICL~\cite{DBLP:conf/acl/HanSMTCW23}{, }\\
                            ROOTS~\cite{DBLP:conf/acl/PiktusAVLDLJR23}{, }
                            QUIP-Score~\cite{DBLP:journals/corr/abs-2305-11859}
                            , leaf, text width=33em
                        ]
                    ]
                    [
                        Out-of-model \\Knowledge  (\S \ref{sec:Out-of-model_Knowledge}), fill=light-skyblue
                        [
                            FiD~\cite{DBLP:conf/eacl/IzacardG21}{,}
                            Retrieval Augmentation~\cite{DBLP:conf/emnlp/0001PCKW21}{, }\\
                            Retro~\cite{DBLP:conf/icml/BorgeaudMHCRM0L22}{, }
                            RR~\cite{DBLP:journals/corr/abs-2301-00303}
                            , leaf, text width=33em
                        ]
                    ]
                ]
                [
                    Datasets (\S \ref{sec:Datasets_for_Attribution}), fill=light-green
                    [
                        WebGPT~\cite{nakano2021webgpt}{, }
                        \sout{WebBrain}~\cite{DBLP:journals/corr/abs-2304-04358}{, }
                        WebCPM~\cite{qin-etal-2023-webcpm}{, }\\
                        CiteBench~\cite{https://doi.org/10.48550/arxiv.2212.09577}{, }
                        ALCE~\cite{gao2023enabling}{, }
                        ExpertQA~\cite{Malaviya2023ExpertQAEQ}{,}\\
                        HAGRID~\cite{hagrid}{, }
                        \sout{SEMQA}~\cite{DBLP:journals/corr/abs-2311-04886}{, }
                        BioKaLMA~\cite{li2023verifiable}
                        , leaf, text width=43em
                    ]
                ]
                [
                    Approaches (\S \ref{sec:Approaches_to_Attribution}), fill=light-green
                    [
                        Direct Generated \\Attribution  (\S \ref{sec:Direct_Generated_Attribution}), fill=light-skyblue
                        [
                            according-to Prompting~\cite{DBLP:journals/corr/abs-2305-11859}{, }
                            CwW~\cite{DBLP:conf/acl/PeskoffS23}{, }\\
                            Attributing Prompting~\cite{zuccon2023chatgpt}{, }IFL~\cite{lee2023towards}{,}\\
                            Blueprint Model~\cite{anonymous2023learning}{, }
                             \sout{1-PAGER}~\cite{DBLP:journals/corr/abs-2310-16568}
                            , leaf, text width=34em
                        ]
                    ]
                    [
                        Post-retrieval \\Answering  (\S \ref{sec:Post-retrieval_Answering}), fill=light-skyblue
                        [
                            SearChain~\cite{DBLP:journals/corr/abs-2304-14732}{, }
                            MixAlign~\cite{DBLP:journals/corr/abs-2305-13669}{, }\\
                            SmartBook~\cite{DBLP:journals/corr/abs-2303-14337}{, }
                            Self-RAG~\cite{DBLP:journals/corr/abs-2310-11511}{, }\\
                            LLatrieval~\cite{li2023llatrieval}{, }
                            AGREE\cite{ye2023effective}
                            , leaf, text width=29em
                        ]
                    ]
                    [
                        Post-Generation \\Attribution  (\S \ref{sec:Post-Generation_Attribution}), fill=light-skyblue
                        [
                            RARR~\cite{DBLP:conf/acl/GaoDPCCFZLLJG23}{, }
                            \sout{SAPLMA}~\cite{DBLP:journals/corr/abs-2304-13734}{, }\\
                            \sout{IQ DQ}~\cite{DBLP:journals/corr/abs-2305-18248}{,}
                            CCVER~\cite{DBLP:journals/corr/abs-2305-11859}{,}\\
                            RSEQGA~\cite{DBLP:journals/corr/abs-2309-11392}
                            , leaf, text width=29em
                        ]
                    ]
                    [
                        Attribution Systems  \\(\S \ref{sec:Attribution_Systems}), fill=light-skyblue
                        [
                            LaMDA~\cite{Thoppilan2022LaMDALM}{, }
                            WebGPT~\cite{nakano2021webgpt}{, }\\
                            GopherCite~\cite{Menick2022TeachingLM}
                            Sparrow~\cite{DBLP:journals/corr/abs-2209-14375}\\
                            \sout{WebCPM}~\cite{qin-etal-2023-webcpm}
                            , leaf, text width=29em
                        ]
                    ]
                ]
                [
                    Evaluation (\S \ref{sec:Attribution_Evaluation}), fill=light-green
                    [
                        \sout{Side}~\cite{DBLP:journals/corr/abs-2207-06220}{, }
                        \sout{Auto-AIS}~\cite{DBLP:conf/acl/GaoDPCCFZLLJG23}{, }
                        \citet{DBLP:journals/corr/abs-2212-08037}{, }
                        \citet{Liu2023EvaluatingVI}{,}\\
                        \sout{WICE}~\cite{DBLP:journals/corr/abs-2303-01432}{, }
                        XOR-AttriQA~\cite{DBLP:journals/corr/abs-2305-14332}{, }
                        \sout{FActScore}~\cite{DBLP:journals/corr/abs-2305-14251}{, }\\
                        AttrScore~\cite{DBLP:journals/corr/abs-2305-06311}{, }
                        FacTool~\cite{DBLP:journals/corr/abs-2307-13528}{, }
                        \citet{DBLP:journals/corr/abs-2309-05217}{, }
                        KaLMA~\cite{li2023verifiable}
                        , leaf, text width=44em
                    ]
                ]
            ]
        \end{forest}
    }
    \caption{Taxonomy of Large Language Models Attribution.}
    \label{taxo_of_icl}
\end{figure*}
